Challenges in Partially-Automated Roadway Feature Mapping Using Mobile Laser Scanning and Vehicle Trajectory Data

Connected vehicle and driver's assistance applications are greatly facilitated by Enhanced Digital Maps (EDMs) that represent roadway features (e.g., lane edges or centerlines, stop bars). Due to the large number of signalized intersections and miles of roadway, manual development of EDMs on a global basis is not feasible. Mobile Terrestrial Laser Scanning (MTLS) is the preferred data acquisition method to provide data for automated EDM development. Such systems provide an MTLS trajectory and a point cloud for the roadway environment. The challenge is to automatically convert these data into an EDM. This article presents a new processing and feature extraction method, experimental demonstration providing SAE-J2735 map messages for eleven example intersections, and a discussion of the results that points out remaining challenges and suggests directions for future research.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Sections/data_old.tex <==

The point cloud data used in this study was collected by the Advanced Highway Maintenance \& Construction Technology Research Center (AHMCT) research center at UC Davis. The data is obtained by scanning Palo Alto testbed along El Camino Real. The Mobile Terrestrial Laser Scanners (MTLS) is a Trimble MX8 which includes two Riegl VQ450 laser scanners and an Applanix POS 520 platform positioning system. The left laser scanner has vehicle relative azimuth, roll and pitch angles of 143, -19 and 23.5 degrees respectively. The right scanner has vehicle relative azimuth, roll and pitch angles of -143, 19 and 23.5 degrees respectively [1]. The platform mounted on the vehicle is shown in Figure \ref{fig:ahmct} . 
%\begin{figure}
%	\begin{center}
%		\begin{tabular}{c}
%			\includegraphics[height=5cm]{ahmct_platform.jpg}
%		\end{tabular}
%	\end{center}
%	\caption[example] 
%	%>>>> use \label inside caption to get Fig. number with \ref{}
%	{ \label{fig:ahmct} 
%		AHMCT MTLS Vehicle. }
%\end{figure} 
The testbed contains 11 signalized intersections. See Table 1. At each intersection, the MTLS platform was driven along each ingress and egress section of the main thoroughfare (El Camino Real) multiple times and along the cross street at least once. The multiple passes along each section provide a dense points cloud on the surface of the street, which will facilitate reliable feature extraction. A second reason for the multiple passes along a road section is that the effect of dynamic obstructions (e.g., other vehicles) is unlikely to be the same in the multiple passes, so their effect is a slightly lower density of returns, instead of the absence of data that would be caused by a single run.  The resulting dataset provides both MTLS georectified point cloud and the trajectory of the platform. The platform trajectory is shown in Fig \ref{fig:preproc1}. The entire point cloud acquired along this trajectory contains approximately 2,560 million points. For each intersection, the J2735 map message requires definition of the intersection center point. This is a designated reference point that should be near the center and later provided in the J2735 map message.  All intersections features described in the J2735 for that intersection will be specified as offsets relative to the defined center. 
Table \ref{size-table} lists the names of the intersection cross streets, the latitude and longitude defined as the center of the intersection, and the number of points within a radius $R = 60$ meters of the intersection center. On average each intersection contains around 80 million points on average. Of the 2,560 million points in the full point cloud, approximately 872 million are within the radius $R$ of at least one of the intersection centers. The remaining 1688 million points are discarded.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
	\centering
	\caption{Point cloud size of the intersections along the Palo-Alto testbed corridor}
	\label{size-table}
	\begin{tabular}{|l|l|l|l|}
		\hline
		\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} \textbf{Cross Street}\\ \textbf{Name}\end{tabular}} & \multicolumn{2}{l|}{\textbf{Center  Coordinates}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{No. of}\\ \textbf{Points}\end{tabular}} \\ \cline{2-3}
		& \textbf{Lat.} & \textbf{Long.} & \\ \hline \hline
		\begin{tabular}[c]{@{}l@{}}Stanford\\ Ave\end{tabular} & 37.4277640 & -122.1492539 & 77.57 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Cambridge\\ Ave\end{tabular} & 37.4255950 & -122.1467851 & 75.36 \\ \hline
		\begin{tabular}[c]{@{}l@{}}California\\ Ave\end{tabular} & 37.4250803 & -122.1458624 & 66.03 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Page Mill\\ Road\end{tabular} & 37.4230638 & -122.1420467 & 95.04 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Portage Ave/\\ Hansen Way\end{tabular} & 37.4210617 & -122.1382334 & 154.58 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Matadero\\ Ave\end{tabular} & 37.4191602 & -122.1345428 & 68.68  \\ \hline
		\begin{tabular}[c]{@{}l@{}}Curtner\\ Ave\end{tabular} & 37.4176288 & -122.1315912 & 70.04 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Ventura\\ Ave\end{tabular}  &  37.4168366 & -122.1300875 & 50.64   \\ \hline
		\begin{tabular}[c]{@{}l@{}}Los Robles\\ Ave\end{tabular}  & 37.4157300 & -122.1281376 & 70.48 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Maybell\\ Ave\end{tabular}  & 37.4120037 & -122.1246158 & 59.78 \\ \hline
		\begin{tabular}[c]{@{}l@{}}Charleston\\ Ave\end{tabular} & 37.4104459 & -122.1233336 & 83.45 \\ \hline
		\multicolumn{3}{|r|}{Total Size} & 871.65 \\ \hline
		\multicolumn{3}{|r|}{Total Data Size}  & 2559.70 \\ \hline
		\multicolumn{3}{|r|}{Discarded Points} & 1688.05 \\ \hline
	\end{tabular}
\end{table}


==> Sections/futurework.tex <==
The details of the feature extraction methodology and its evaluation on eleven intersections demonstrate the complexity of representing relevant roadway features in a standard usable format within a connected vehicle environment. The algorithm worked well in spite of these complexities, making a significant advance from manual feature extraction toward automated data processing for roadway relevant feature extraction. Following are a few avenues fruitful for future efforts:
\begin{enumerate}
	\item Automated feature extraction advancements are developed best within an application testbed environment. UCR is interested in collaborating with government agencies, academic groups, or commercial entities in testbed applications and demonstration projects that require roadway relevant maps and allow the opportunity for advancements within the automated mapping field.
	\item The accuracy of roadway feature maps is built upon the foundation of the platform trajectory estimation step in the georectification process. Methods to enhance the reliability and integrity of high accuracy, especially in GNSS challenged environments is necessary.
	\item The approach presented herein was limited in scope to intersections and specific features. Broadening this is important. 
\end{enumerate}
	
Evolution of geospatial data acquisition will yield ever increasing accurate and precise topology data for the roadway environment. The necessity to identify and extract relevant roadway features will become significantly more valuable. The methodology presented herein focused on roadway attributes associated with intersection relevant road surface features. It should be viewed as a glimpse of what is possible in the future as the technology develops. Present and future sensing and computing resources are not the limiting factors. This field is in its infancy. Feature extraction algorithms, mapping standards, commercial approaches, and potential connected vehicle applications are still in their formative and demonstration phases. 

